Experimental Study on the Effect of Synchronization Accuracy for Near-Field RF Wireless Power Transfer in Multi-Antenna Systems

Wireless power transfer (WPT) technologies hold promise for enhancing device autonomy, particularly for energy-limited IoT systems. This paper presents experimental results on coherent and non-coherent transmit diversity approaches for WPT, tested in the near field using the Techtile testbed. We demonstrate that a fully synchronized beamfocusing system achieves a 14 dB gain over non-coherent transmission, consistent with the theoretical 14.9 dB gain for a 31-element array. Additionally, phase alignment errors below 20{\deg} result in less than 1 dB of gain loss, while errors exceeding 40{\deg} lead to losses over 3 dB. These findings suggest that phase coherency requirements for WPT can be relaxed, and that scaling the number of antennas is a promising strategy for improving power transfer efficiency.

==> figures/techtile/non-coherent/partial-power-tx.tex <==
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={M},
xmajorgrids,
xmin=-3.1, xmax=87.1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Power [W]},
ymajorgrids,
ymin=3.95, ymax=5.4,
ytick style={color=black}
]


\draw[black, semithick,fill=black!5, fill opacity=0.8] (2,4.06) rectangle (84,4.24); %



\addplot [semithick, steelblue31119180] table [col sep=space, x=x, y=y] {figures/techtile/non-coherent/partial-power-tx.dat};


\draw[black, semithick] (2,0.92) -- (21,1.132); %

\draw[black, semithick] (84,0.92) -- (78.8,1.132); %


\end{axis}

 \begin{axis}[xmin=2,xmax=84,ymin=4.06,ymax=4.24,grid,height=4cm,width=6cm,
            shift={(1.8cm,2.5cm)},axis background/.style={fill=black!3}]
            \addplot[semithick, steelblue31119180] table [col sep=space, x=x, y=y] {figures/techtile/non-coherent/partial-power-tx.dat};
\end{axis}            

\end{tikzpicture}

